Sensitivity Oracles for All-Pairs Mincuts

Let $G=(V,E)$ be an undirected unweighted graph on $n$ vertices and $m$ edges. We address the problem of sensitivity oracle for all-pairs mincuts in $G$ defined as follows. Build a compact data structure that, on receiving any pair of vertices $s,t\in V$ and failure (or insertion) of any edge as query, can efficiently report the mincut between $s$ and $t$ after the failure (or the insertion). To the best of our knowledge, there exists no data structure for this problem which takes $o(mn)$ space and a non-trivial query time. We present the following results. - Our first data structure occupies ${\cal O}(n^2)$ space and guarantees ${\cal O}(1)$ query time to report the value of resulting $(s,t)$-mincut upon failure (or insertion) of any edge. Moreover, the set of vertices defining a resulting $(s,t)$-mincut after the update can be reported in ${\cal O}(n)$ time which is worst-case optimal. - Our second data structure optimizes space at the expense of increased query time. It takes ${\cal O}(m)$ space -- which is also the space taken by $G$. The query time is ${\cal O}(\min(m,n c_{s,t}))$ where $c_{s,t}$ is the value of the mincut between $s$ and $t$ in $G$. This query time is faster by a factor of $\Omega(\min(m^{1/3},\sqrt{n}))$ compared to the best known deterministic algorithm to compute a $(s,t)$-mincut from scratch. - If we are only interested in knowing if failure (or insertion) of an edge changes the value of $(s,t)$-mincut, we can distribute our ${\cal O}(n^2)$ space data structure evenly among $n$ vertices. For any failed (or inserted) edge we only require the data structures stored at its endpoints to determine if the value of $(s,t)$-mincut has changed for any $s,t \in V$.

==> src/old_sections.tex <==
\subsubsection{Query Transformation}
The aim of this section is to study some properties of $(u,v)$-mincut which help us to transform a query procedure to another equivalent query. Remember, the query we have is of the form $Q(u,v,E_y)$ on graph $G$ in which we need to report if all edges in $E_y$ lie in some $(u,v)$-mincut. Another set of edges from graph $G$, say $E'$, not necessarily having common end point is obtained, which satisfies the property that all edges in $E_y$ lie in some $(u,v)$-mincut if and only if all edges in $E'$ lie in some $(u,v)$-mincut.

One might question the relevance of such a transformation for our use. We will make use of this transformation to get a set of edges $E'$ which have the following property,
~(i) their endpoints are different vertices in $G_\nu$, and
~(ii) all the edges in $E'$ share a common end point in $G_\nu$. This will enable us to transform a query $Q(u,v,E_y)$ on $G$ to an equivalent query $Q(u,v,E')$ on $G_\nu$.

% {\color{red} SODA2021-alternate import begin}

%%%%%%%Query transformation lemma begin

Let $r,s,t$ be any three vertices from $S$
and let $A\subset V$ define a steiner mincut that separates $\{r,s\}$ from $t$. Recall that strip ${\cal W}_A$ stores all $(s,t)$-mincuts that enclose $A$. Our aim is to investigate the properties of a $(r,s)$-mincut with respect to the strip ${\cal W}_A$.

Let $B$ be any $(r,s)$-mincut. If $B\subseteq A$, all vertices presents in the nodes ${\cal W}_A\backslash {\mathbf{s}}$ appear on one side of the $(r,s)$-mincut. So let us consider the more interesting case in which $B$ crosses $A$. Firstly, it follows from Lemma \ref{lem:B-crosses-A} that each node of the strip ${\cal W}_A$, excluding of course $\mathbf{s}$, remain intact in each $(r,s)$-mincut. This suggests that we can replace the subgraph of $G$ induced by $\bar{A}$ by the strip ${\cal W}_A$ above ${\mathbf{s}}$. Alternatively, we blow-up the node $\mathbf{s}$ of ${\cal W}_A$ into the subgraph induced by the vertices assigned to it. We call this graph $G_A$ henceforth. The following figure illustrates ${\cal W}_A$ and $G_A$.

\begin{figure}[h]
    \centering
    \includegraphics[width=0.9\textwidth]{src/images/G_A.png}{}
    \caption{Suitable caption to be added}
    \label{fig:G_A}
\end{figure}

Let $y$ be any non-terminal unit in strip ${\cal W}_{A}$. Let $x_1,\ldots,x_k$ be any $k$ neighbors of $y$. In case all the neighbours are on the side of $\mathbf{s}$, let $R$ be the union of their reachability cones, on the side of $\mathbf{s}$, excluding the terminal ${\mathbf{s}}$. In case all neighbours are on the side of $\mathbf{t}$, consider $R$ to be the reachability cone of $y$ on the side of $\mathbf{s}$ excluding the terminal $\mathbf{s}$.

We know that there exists a $(s,t)$-mincut that cuts edges $(y,x_i)$ for each $1\le i \le k$. There also exists a $(s,t)$-mincut that cuts all edges emanating from $R$ on the side of $\mathbf{s}$. What about the $(r,s)$-cut defined by $B$ that crosses $A$. We shall show an important claim on the following page. The intuition underlying the claim is as follows. 

For each $(r,s)$-cut that crosses $A$, we can associate a $(r,t)$-mincut that encloses $A$. Since the latter is a transversal on ${\cal W}_A$, this allows us to exploit properties of ${\cal W}_A$ stated in 
Lemma \ref{lem:reachability-cone-in-W-st} and Corollary
\ref{cor:1-W_A-2-nearest-mincut}. This helps us in deriving inferences for the cut defined by $B$.

\begin{lemma}
\label{lem:reachability-cone-u-v-mincut}
There is a $(r,s)$-mincut that cuts edges $\{(y,x_1),\ldots, (y,x_k)\}$ if and only if there is a $(r,s)$-mincut that cuts all edges emanating from $R$ on the side of $\mathbf{s}$.
\end{lemma}
\begin{proof}
Let all $x_i's$ be on the side of $\mathbf s$ from $y$. The proof for other side will follow likewise.

Let $B$ be a $(r,s)$-mincut that cuts edges $\{(y,x_1),…,(y,x_k)\}$. 
Refer to Figure \ref{fig:B-crosses-A}($i$).
Observe that $y$ does not belong to $A$. So $A\cup B$ also cuts edges $\{(y,x_1),…,(y,x_k)\}$, and $\{x_1,\ldots,x_k\}$ belong to $A\cup B$.
It follows from  Lemma \ref{lem:B-crosses-A} (ii) that $A\cup B$ is a $(r,t)$-mincut. Since $A\cup B$ encloses $A$, so
$A\cup B$ must be a transversal on ${\cal W}_A$.  Therefore,
$R$ belongs to $A\cup B$.
%Applying Corollary \ref{cor:1-W_A-2-nearest-mincut}(2), it follows that the nearest mincut between $\{r,x_1,…,x_k\}$ and $t$ must contain $R$. 
%Since $x_i$’s belong to $A\cup B$, it follows that $A\cup B$ is also a mincut between $\{r ,x_1,…,x_k\}$  and $t$. 
%So $R$ belongs to $A\cup B$ as well.
It follows from the construction that $R$ lies totally outside $A$, that is, $R\cap A=\emptyset$. Therefore, since
$R$ belongs to $A\cup B$, $R$ must lie fully inside $\bar{A}\cap B$. 
Using this fact and Lemma \ref{lem:B-crosses-A} (iii), all edges emanating from $R$ on the side of $\mathbf{s}$
are incident only on $A\cap B$. But $A\cap B$ defines a $(r,s)$-mincut as follows from Lemma \ref{lem:B-crosses-A} (i). 
%This cut is obtained by removing $\bar{A}\cap B$ from $B$. So it follows that $R$ lies outside $A\cap B$ and $R$ contributes all outgoing edges to the cut defined by $A\cap B$. 
So $A\cap B$ defines the desired $(r,s)$-cut.
\begin{figure}[h]
    \centering
    \includegraphics[width=0.9\textwidth]{src/images/B-crosses-A.png}{}
    \caption{($i$) $B$ cuts edges $\{(y,x_1),\ldots,(y,x_k)\}$.~$(ii)$ $B$ cuts all outgoing edges of $R$.}
    \label{fig:B-crosses-A}
\end{figure}

Let $B$ be a $(r,s)$-mincut with that cuts all edges emanating from $R$ on the side of $\mathbf{s}$. Refer to Figure \ref{fig:B-crosses-A}($ii$). By construction $R$ lies outside $A$, and the cut defined by $A$ cuts all edges emanating from $R$ on the side of $\mathbf{s}$.
 Therefore, the cut defined by $A\cup B$ cuts all edges emanating from $R$ on the side of $\mathbf{s}$. Using Lemma \ref{lem:B-crosses-A} (ii), $A\cup B$ is a $(r,t)$-mincut. Since each $(r,t)$-mincut that encloses $A$ is a transversal on ${\cal W}_A$, it follows that $(A\cup B) \cap R = \emptyset$. So $B \cap R = \emptyset$ too. That is, $R$ lies entirely on the side of $t$ in the cut defined by $B$. Treating $R$ as a single vertex, observe that its incoming edges are the same in number as its outgoing edges. It is given that $R$ currently contributes all its outgoing edges to the cut defined by $B$. So it follows that $B\cup R$ has the same capacity as $B$ and $R$ now contributes all incoming edges to the cut defined by $B \cup R$. Now observe that $r$ belongs to $B\cup R$ since $r$ is in $B$ by construction. $s$ does not belong to $B \cup R$ since, by construction, $s$ is neither in $R$ nor in $B$. So  $B\cup R$ is a $(r,s)$-mincut. It follows from above that all incoming edges of $R$ contribute to this cut. So the cut defined by $B\cup R$ cuts all edges $(y,x_1),…,(y,x_k)$. So $B\cup R$ is the desired $(r,s)$-cut.
\end{proof}

%%%% Query transformation lemma end %%%%
% {\color{red} SODA2021-alternate import end}




\subsection{Construction of compact graph for any $S\subseteq V$}
{\color{red} Correct cycles to cycles/tree edges}
The contraction procedure is pretty much the same as in the contraction at root node. The only difference is caused by stretched units as they are mapped to a proper path in the skeleton ${\cal H}_S$ rather than a single node. The construction of $G_\nu$ is as follows.

Let us fix any arbitrary total order on the cycles and tree edges in skeleton ${\cal H}_S$. It is important to note that the ordering is same for cycles and tree edges. The construction of $G_\nu$ is as follows. We keep all the vertices mapped to node $\nu$ in the skeleton as it is in $G_\nu$ (call them $V_\nu$). We create $j = |C_\nu|+|E_\nu|$ vertices, one for each of the $j$ cycles and tree-edges in the set $C_\nu \cup E_\nu$. Since, we have a total order on all cyles and tree edges. We can assume that $C_\nu \cup E_\nu$ is an ordered set. The $\ell^{th}$ element of this set be denoted by $e_\ell$. Let $c_\ell$ denote the vertex corresponding to $e_\ell$. Consider any vertex $v\notin V_\nu$. Let the unit, it belongs to, be mapped to  $P(\nu_1,\nu_2)$. We assign $v$ to one of $\{c_1,\ldots,c_j\}$ as follows.
\begin{itemize}
    \item If $\nu_1=\nu$ and $\nu_2\in {\cal H_S}(e_i)$, $v$ is assigned to $c_i$. Moreover, if  $\nu_1\in {\cal H_S}(e_i)$ and $\nu_2=\nu$, $v$ is assigned to $c_i$.
    \item If $\nu_1 \in {\cal H_S}(e_i)$ and $\nu_2\in {\cal H_S}(e_k)$, $v$ is assigned to $c_{\min(i,k)}$
\end{itemize}

\noindent

\begin{figure}[h]
    \centering
    \includegraphics[width=1.0\textwidth]{src/images/image_contraction.pdf}{}
    \caption{Contraction procedure. We only show the vertices of graph, some edges of graph and the skeleton ${\cal H}_S$. Solid vertices belong to steiner set $S$ and hollow vertices are non-steiner vertices. Blue edges denote some of the graph edges.}
    \label{fig:image-contraction}
\end{figure}

Let us focus on cycle $C_i$ for any $i\le j$. Let $e_1$ and $e_2$ be the structural edges in this cycle that are incident on node $\nu$. Let ${\cal W}$ be the strip corresponding to the subbunch formed by these two structural edges. Let $\mathbf s$ and $\mathbf t$ be the source and sink of this strip respectively. Also, assume that $\nu$ is on the side of source. We now state a lemma that states an important property about $G_\nu$.

\begin{lemma}
Let $u$ be a non-terminal unit in ${\cal W}$. Let $u'$ be any unit reachable from $u$ in the direction of ${\mathbf{s}}$. $u'$ will be compressed to the same cycle node as $u$ during the construction of $G_\nu$.
\label{lem:u-u'-in-G-nu}
\end{lemma}
\begin{proof}
Let the proper paths associated with each of $u$ and $u'$ in ${\cal H}_S$ be $P(\nu_1,\nu_2)$ and $P(\nu_3,\nu_4)$ respectively. 
It follows from the construction of ${\cal W}$ that
$P(\nu_1,\nu_2)$ as well as $P(\nu_3,\nu_4)$ will pass through either structural edge $e_1$ or structural edge $e_2$. Without loss of generality,  assume that $P(\nu_1,\nu_2)$ passes through $e_1$. Since both $e_1$ as well as $e_2$ belong to $C_i$ and $P(\nu_1,\nu_2)$ is a proper path, this would imply that it will not pass through $e_2$. Since $u'$ is reachable from $u$, so $P(\nu_3,\nu_4)$ will also have to pass through $e_1$.
It follows from Corollary \ref{th:reachability-cone-proper-path}, that 
$P(\nu_1,\nu_2)$ as well as $P(\nu_3,\nu_4)$ are subpaths of a path, say $P(\nu',\nu'')$, in skeleton
${\cal H}_S$. This combined with the above discussion establishes that $P(\nu',\nu'')$ has the structure shown in Figure \ref{fig:structure-of-p(nu',nu'')}.

Observe that any path in skeleton that passes through a node $\nu$ can intersect at most 2 cycles that are passing though $\nu$. We know that prefix of $P(\nu',\nu'')$ upto $e_1$ pass through $C_i$, so the suffix can pass through exactly one cycle $C_\ell, \ell \not=i$.
Since $\nu_2$ and $\nu_4$ belong to the compressed node of $C_j$. This completes the proof.
\end{proof}


\begin{lemma}
Let $A_i$ be the set of vertices compressed to $c_i$. The cut $(A_i,\bar{A_i})$ represent a Steiner mincut from strip ${\cal W}$.
\end{lemma}
\begin{proof}
Let $U_k$ be the set of non-terminal units in strip ${\cal W}$ such that the proper path to which it is mapped has one end point in cycle $C_k$. We already know that the other end point is in cycle $C_i$ since this unit appears as a non-terminal in the strip. Consider the cut defined by 
$\cup_{k\not=i} U_k \cup {\mathbf{s}}$.
It follows from Lemma \ref{lem:u-u'-in-G-nu} that 
${\cal R}_{\mathbf s}(U_k) \setminus {\mathbf s} = U_k$.
Therefore, $\cup_{k\not=i} U_k \cup {\mathbf{s}}$ is a transversal on ${\cal W}$, and hence is a Steiner mincut.
\end{proof}


% As evident from the results of \cite{DBLP:journals/mp/PicardQ82}, the number of $(u,v)$-mincuts can be exponential for a designated source and sink vertex. The query $Q(u,v,E_y)$ on graph $G$ requires to check if all edges in $E_y$ lie in some $(u,v)$-mincut. This means that we somehow have to check the presence of these edges in all the $(u,v)$-mincuts. The aim of constructing $G_\nu$ is to preserve as many $(u,v)$-mincuts as possible in a smaller compact graph. However, there may be some $(u,v)$-mincuts in $G$ which are missing in $G_\nu$. To circumvent this problem we transform a query $Q(u,v,E_y)$ on $G$ in such a way that it can be answered from the $(u,v)$-mincuts in $G_\nu$ itself.

% {\color{blue} Revised version ends}



% {\color{red} Old version begins}


% In this section, we will discuss the \textit{contraction procedure}, i.e. obtaining $G_\nu$ from graph $G$ and connectivity carcass $\mathfrak{C}_S$. Thereafter, we establish more formally how $G_\nu$ preserves the connectivity of steiner vertices mapped to node $\nu$.

% \subsubsection{Contraction procedure}
% To accomplish the contraction procedure, we define an order on the cycles. The ordering can be done arbitrarily. Since, $G_\nu$ is a quotient graph of $G$ it can be obtained from $G$ by applying certain vertex contractions. We keep all the vertices mapped to node $\nu$ in the skeleton as it is in $G_\nu$ (call them $V_\nu$). We create a vertex corresponding to each cycle (call them cycle vertices) passing through $\nu$ in new graph $G_\nu$. Now, for each vertex mapped to $P(\nu_1,\nu_2)$ (not $P(\nu,\nu)$) the contraction proceeds as follows,
% \begin{itemize}
%     \item If $P(\nu_1,\nu_2)$ does not pass through $\nu$, then it is contracted to the vertex corresponding to the cycle in which this path completely lies,
%     \item if $P(\nu_1,\nu_2)$ has one end point as $\nu$, then it is contracted to the vertex corresponding to the cycle in which its second end-point lies,
%     \item if $P(\nu_1,\nu_2)$ passes through $\nu$ but does not have it as an end-point, the unit is contracted to the cycle vertex corresponding to lesser ordered cycle.
% \end{itemize}

% \noindent
% Let $C_1,C_2,...,C_j$ be the cycles in the skeleton which pass through node $\nu$. Let us focus on cycle $C_i$. Let $e_1$ and $e_2$ be the structural edges in this cycle that are incident on node $\nu$. Let ${\cal W}$ be the strip corresponding to the bunch formed by these two structural edges. Let $\mathbf s$ and $\mathbf t$ be the source and sink of this strip respectively. Also, assume that $\nu$ is on the side of source.

% Let $U_k$ be the set of non-terminal units in this strip such that the proper path to which it is mapped has one end point in cycle $C_k$ (not $\nu$ although). We already know that the other end point is in cycle $C_i$ since this unit appears as a non-terminal in the strip. Let $\mathbf u \in U_i$ be a non-terminal unit. Using \ref{th:reachability-cone-proper-path}, it is evident that all non-terminal units in ${\cal R}_{\mathbf s}(\mathbf u) \setminus {\mathbf s}$ belong to set $U_i$. Overloading the notation, let ${\cal R}_{\mathbf s}(U_k) \setminus {\mathbf s}$ represents the union of ${\cal R}_{\mathbf s}(\mathbf u) \setminus {\mathbf s}$ $\forall\; {\mathbf u}\in U_k$. This simple property leads to the following,

% \begin{equation}
%     \begin{split}
%         \nonumber
%         {\cal R}_{\mathbf s}(U_k) \setminus {\mathbf s} &= U_k \\
%         \implies \bigcup_{k<i}{\cal R}_{\mathbf s}(U_k) \setminus {\mathbf s} &= \bigcup_{k<i} U_k
%     \end{split}
% \end{equation}

% Thus, the set $\bigcup_{k<i} U_k$ forms a closed set in the strip ${\cal W}$. Consider a transversal $(A,{\bar A})$ such that $A$ contains all the units in $\bigcup_{k<i} U_k$ as well as source $\mathbf{s}$. It is evident that $(A,{\bar A})$ is also a steiner mincut.


% % As evident from the results of \cite{DBLP:journals/mp/PicardQ82}, the number of $(u,v)$-mincuts can be exponential for a designated source and sink vertex. The query $Q(u,v,E_y)$ on graph $G$ requires to check if all edges in $E_y$ lie in some $(u,v)$-mincut. This means that we somehow have to check the presence of these edges in all the $(u,v)$-mincuts. The aim of constructing $G_\nu$ is to preserve as many $(u,v)$-mincuts as possible in a smaller compact graph. However, there may be some $(u,v)$-mincuts in $G$ which are missing in $G_\nu$. To circumvent this problem we transform a query $Q(u,v,E_y)$ on $G$ in such a way that it can be answered from the $(u,v)$-mincuts in $G_\nu$ itself.

% {\color{red} Old version ends}

We establish the following lemma which presents the results of Lemma \ref{lem:small-graph-equivalent-S=V} in a more general form.

\begin{lemma} \label{lem:small-graph-equivalent}
Let $G_\nu$ be the graph corresponding to node $\nu$ in skeleton ${\cal H}_S$, obtained from graph $G$ and connectivity carcass $\mathfrak{C}_S$ using the \textit{contraction procedure}. If $u,v \in V_\nu \cap S$,
\begin{enumerate}
    \item For any $(u,v)$-mincut in $G$, there exists a $(u,v)$-mincut in $G_\nu$ that defines the same $2-$partition of set $V_\nu$. Moreover, the value of $(u,v)$-mincut remains same in both $G$ and $G_\nu$.
    \item Let $E' \subset E$ be a set of edges whose endpoints are contracted to different vertices in $G_\nu$. There is a $(u,v)$-mincut in $G$ that cuts all edges in $E'$, if and only if there is a $(u,v)$-mincut in $G_\nu$ that cuts all edges in $E'$.
\end{enumerate}
\end{lemma}
\begin{proof}
Let $c_1,c_2,...,c_j$ be the cycle vertices in $G_\nu$ corresponding to cycles $C_1,C_2,...,C_j$ of skeleton $\mathcal H_S$. It is also known that $\nu$ is part of all these cycles.

Consider $(A_i,\overline A_i)$ to be a cut in $G$ that keeps all vertices contracted to $c_i$ on side $\overline A_i$ and all the other vertices in $A_i$. We have already argued that each of the cuts $(A_i, \overline A_i)$ form a steiner mincut.

Given a $(u,v)$-mincut ${\cal C}=(B,{\bar B})$ that cuts all edges in $E'$ it suffices to construct another $(u,v)$-mincut ${\cal C}'=(B',{\bar B'})$ that cuts all edges in $E'$ and keeps all the vertices of ${\bar A_i}$ on one side $\forall i \in [j]$. It is clear that such a mincut will also be present in $G_\nu$.

For each set $A_i$, where $i\in [j]$ repeat the following procedure. If $B$ keeps ${\bar A_i}$ on one side proceed to next $i$. Otherwise, if $B\cap {\bar A_i}$ (or ${\bar B}\cap {\bar A_i}$) consists of some steiner vertices then replace the $(u,v)$-mincut $(B,{\bar B})$ by $(u,v)$-mincut $({\bar A_i}\cup B,A_i\cap {\bar B})$ (or $(A_i\cap B,{\bar A_i}\cup {\bar B})$) and proceed to next $i$.

It is clear that following the above procedure we eventually get a $(u,v)$-mincut that keeps all the vertices of ${\bar A_i}$ on one side $\forall i \in [j]$. This $(u,v)$-mincut will define the same partition in $V_\nu$. Moreover, it will also cut all edges in $E'$.

The above result also implies that the value of $(u,v)$-mincut in $G$ is same as that in $G_\nu$ for any $u,v \in V_\nu \cap S$. Thus, the other direction of both the proofs are trivial.
\end{proof}

Again, the above lemma implies that a query $Q(u,v,E')$ on $G$ will produce the same outcome on $G_\nu$ provided that all edges in $E'$ have distinct end points in $G_\nu$. Similar to the base case, we use the notion of query transformation to deal with the  edges whose end point are contracted to single vertex in $G_\nu$. Thus, we arrive at the following lemma that presents our key insight in the most concise form.

\begin{lemma} \label{lem:edge-correspondence}
Let $u,v \in S$ mapped to same node $\nu$ in skeleton $\mathcal H_S$ corresponding to graph $G$ and steiner set $S\subseteq V$. For a given set of edges $E_y$ emanating from a given vertex $y$ in $G$, there exists a set of edges $E_{y'}$ emanating from a vertex $y'$ in $G_\nu$ such that $E_y$ lies in a $(u,v)$-mincut in $G$ if and only if $E_{y'}$ lies in a $(u,v)$-mincut in $G_\nu$. Set of edges $E_{y'}$ can be obtained from $E_y$ given flesh $\mathcal F_S$ and skeleton $\mathcal H_S$ in time linear in the size of flesh.
\end{lemma}

\begin{proof}
First of all we consider the case when $y$ is mapped to $\nu$. In this case, all the edges of $E_y$ are also present in $G_\nu$. Using Lemma \ref{lem:small-graph-equivalent}(ii), it is clear that the proposition holds taking $y'=y$ and $E_{y'}=E_y$.

% Now, consider the case when $y$ is contracted to some cycle node $c$ in $G_\nu$. Assume that cycle node $c$ corresponds to cycle $C$ in the skeleton ${\cal H}_S$. Consider $(A,{\bar A})$ to be the steiner mincut in graph $G$ such that ${\bar A}$ consists of all the vertices contracted to cycle node $c$. Also consider a $(u,v)$-mincut $(B,{\bar B})$ that cuts all edges in $E_y$. Based upon whether the cut $(B,{\bar B})$ $S-$crosses the cut $(A,{\bar A})$ one of the cases from Lemma \ref{lem:crossing-and-non-crossing-steiner-mincut} may arise. Without loss in generality, it can be assumed that $B\cap {\bar A}$ contains atleast a steiner vertex. It can be observed that in either of the cases ${\bar A}\cap B$ defines a steiner mincut. Since, this steiner mincut cuts all edges in $E_y$, they must be in the same side of the inherent partition of $y$. 

% Now, consider the case when $y$ is contracted to some cycle node $c$ in $G_\nu$. Assume that cycle node $c$ corresponds to cycle $C$ in the skeleton ${\cal H}_S$. Consider $(A,{\bar A})$ to be the steiner mincut in graph $G$ such that ${\bar A}$ consists of all the vertices contracted to cycle node $c$. Also consider a $(u,v)$-mincut $(B,{\bar B})$ that cuts all edges in $E_y$. Based upon whether the cut $(B,{\bar B})$ $S-$crosses the cut $(A,{\bar A})$ one of the cases from Lemma \ref{lem:crossing-and-non-crossing-steiner-mincut} may arise. Without loss in generality, it can be assumed that $B\cap {\bar A}$ contains atleast a steiner vertex. It can be observed that in either of the cases ${\bar A}\cap B$ defines a steiner mincut. Since, this steiner mincut cuts all edges in $E_y$, they must be in the same side of the inherent partition of $y$. 

Consider $(A,{\bar A})$ to be the steiner mincut in graph $G$ such that ${\bar A}$ consists of all the vertices contracted to cycle node $c$.

Let unit mapped to node $\nu$ be $U$ and thus $u,v\in U$. Consider \textit{any} steiner unit $U_1 \notin A$ mapped to node $\nu_1$. Construct the strip ${\cal W}$ containing all steiner mincuts separating $U$ from $U_1$. If there exists any $(u,v)$-mincut $B$ that cuts all edges in $E_y$, then all edges in $E_y$ must appear in the strip. This is because if $U_1 \in B$ (wlog) then ${\bar A}\cap B$ must be a steiner mincut (from Lemma \ref{lem:crossing-and-non-crossing-steiner-mincut} (i)) separating $U_1$ from $U$ and also cutting all edges in $E_y$.

Using Lemma \ref{lem:reachability-cone-u-v-mincut}, we can obtain another set of edges $E_{y'}$ that have one end point in ${\bar A}$ and other end point in $A$, and also satisfy the property that all edges in $E_y$ lie in some $(u,v)$-mincut ${\cal C}$ in $G$ if and only if all edges in $E_{y'}$ lie in some $(u,v)$-mincut ${\cal C}'$ of $G$. Moreover, using \ref{lem:small-graph-equivalent} (ii) we can argue that this can happen if and only if there exists a $(u,v)$-mincut in $G_\nu$ that cuts all edges in $E_{y'}$. Final thing to observe is that all edges in $E_{y'}$ do emanate from a single vertex $y'=c$ in graph $G_\nu$. This completes the proof for first part.

% Let $y$ be a stretched unit in the skeleton. Assume the proper path to which it is mapped in skeleton ${\cal H}_S$ be $P(\nu_1,\nu_2)$. Consider the paths $(\nu,\nu_1)$,$(\nu,\nu_2)$ and $(\nu_1,\nu_2)$ in the tree ${\cal T}({\cal H}_S)$. Atleast one of the paths $(\nu,\nu_1)$ or $(\nu,\nu_2)$ must intersect the path $(\nu_1,\nu_2)$. Let $(\nu,\nu_1)$ be one such path. Consider the strip consisting of all mincuts between node $\nu_1$ and node $\nu$. Since, $y$ appears as a non-terminal in this strip, it is clear that all edges in $E_y$ must be present in this strip. Moreover,$A$ will appear as a transversal in this strip. Using Lemma \ref{lem:reachability-cone-u-v-mincut}, we can obtain another set of edges $E_{y'}$ that have one end point in ${\bar A}$ and other end point in $A$, and also satisfy the property that all edges in $E_y$ lie in some $(u,v)$-mincut ${\cal C}$ in $G$ if and only if all edges in $E_{y'}$ lie in some $(u,v)$-mincut ${\cal C}'$ of $G$. Moreover, using \ref{lem:small-graph-equivalent} (ii) we can argue that this can happen if and only if there exists a $(u,v)$-mincut in $G_\nu$ that cuts all edges in $E_{y'}$. Final thing to observe is that all edges in $E_{y'}$ do emanate from a single vertex $y'=c$ in graph $G_\nu$. This completes the proof for first part.

% Let $y$ is a terminal unit and mapped to node $\nu_1$. We can again accomplish the procedure by constructing the strip ${\cal W}$ consisting of all mincuts between node $\nu_1$ and $\nu$. However, the explanation is slightly different in this case. Assume that $B$ does not $S-$cross $A$. In this case, all the units in ${\bar A}\cap {\bar B}$ are stretched units. Thus, $y$ must lie in ${\bar A}\cap B$. Clearly, ${\bar A}\cap B$ is a steiner mincut that separates $y$ from $\nu$. Thus, all edges in $E_y$ must be present in the strip ${\cal W}$. Same observation can be made in the case when $B$ $S-$crosses $A$. If all edges in $E_y$ are present in ${\cal W}$, the remaining proof is same as above. Now, it is quite possible that all edges in $E_y$ are not present in strip ${\cal W}$. We have already shown that this implies that all edges in $E_y$ cannot lie in any $(u,v)$-mincut. The lemma trivially holds in this case as well.


% Observe the proper path to which any edge in $E_y$ is mapped in the skeleton. Foremost property to observe is that all these proper paths must be extendable to a bigger proper path which can intersect cycle $C$ at atmost one structural edge. It can be shown that all edges in $E_y$ must be mapped to a proper path that intersects cycle $C$ at a structural edge. 

% Consider the case when $B$ does not $S-$crosses $A$. It is clear that the steiner mincuts $A$ and $A\cap {\bar B}$ define the same $2-$partition of the steiner set and hence, belong to same bunch. Since the cut $(A,{\bar A})$ is induced by two structural edges of $C$ incident on $\nu$ (say $e_1,e_2$), the cut $(A\cap {\bar B},{\bar A}\cup B)$ must be induced by the same two structural edges. This means that all the edges in $E_y$ must be mapped to a proper path that intersects cycle $C$ at structural edges $e_1$ or $e_2$. Consider the other case when $B$ $S$-crosses $A$. It this case, from Lemma \ref{lem:crossing-and-non-crossing-steiner-mincut} (ii) it follows that all the three cuts $A$, ${\bar A}\cap B$ and ${\bar A}\cap {\bar B}$ are steiner mincuts and define a partition on the vertex set $V$. Moreover, $A$ is induced by two structural edges $(e_1,e_2)$ in $C$  incident on $\nu$. Using Lemma \ref{lem:3-partition-from-cycle}, we can argue that the other two cuts also arise from same cycle. Let $e_3$ be the other structural edge in the cycle $C$, such that cuts  ${\bar A}\cap B$ and ${\bar A}\cap {\bar B}$ are induced by edges $(e_1,e_3)$ and $(e_2,e_3)$ respectively. Since, all edges in $E_y$ are cut by both these cuts, it is clear that all edges in $E_y$ must be mapped to proper paths which intersects cycle $C$ at structural edge $e_3$.

% Henceforth, we assume that-
% ~(i) $E_y$ lie in same inherent partition of $y$ in flesh ${\cal F}_S$, and
% ~(ii) all edges in $E_y$ are mapped to proper paths which intersect cycle $C$ at structural edges $e_1,e_2$ or some other structural edge $e_3$ of skeleton ${\cal H}_S$. Violating any of the above conditions implies that there is no $(u,v)$-mincut that can cut all edges in $E_y$.

% Consider $e$ to be one of the structural edge of cycle $C$ to which all edges in set $E_y$ are mapped. Let $\mu$ ($\neq \nu$) be one end point of structural edge $e$. Consider the $(\pi^{-1}(\mu),\pi^{-1}(\nu))$ strip storing all mincuts separating vertices mapped to $\mu$ from those mapped to $\nu$. We know that cut $A$ will appear as a transversal in this strip. Moreover, $y$ must appear outside this transversal in the strip. Using Lemma \ref{lem:reachability-cone-u-v-mincut}, we can obtain another set of edges $E_y'$ that have one end point in ${\bar A}$ and other end point in $A$, and also satisfy the property that all edges in $E_y$ lie in some $(u,v)$-mincut ${\cal C}$ in $G$ if and only if all edges in $E_{y'}$ lie in some $(u,v)$-mincut ${\cal C}'$ of $G$. Moreover, using \ref{lem:small-graph-equivalent} (ii) we can argue that this can happen if and only if there exists a $(u,v)$-mincut in $G_\nu$ that cuts all edges in $E_{y'}$. Final thing to observe is that all edges in $E_{y'}$ do emanate from a single vertex $y'=c$ in graph $G_\nu$. This completes the proof for first part.

Obtaining the edges $E_{y'}$ can be done by
~(i) constructing the strip ${\cal W}$ storing all steiner mincuts separating $U$ and $U_1$,
~(ii) computing multiple reachability cones in this dag to obtain $E_{y'}$. Each of these procedures can be carried out in time linear to the size of flesh graph ${\cal F}_S$.
\end{proof}



Using \ref{lem:edge-correspondence}, it is easy to observe that query $Q(u,v,E_y)$ in $G$ is equivalent to the query $Q(u,v,E_{y'})$ on $G_\nu$. We will use this construction of $G_\nu$ to build our ${\cal O}(m)$ size data structure. Furthermore, it will be shown that the query procedure on this data structure which uses multiple query transformations takes ${\cal O}(\min(m,nc_{uv}))$ time in total.

==> src/review.tex <==
\begin{table}
\centering
\begin{tabular}{llll}
\textcolor[rgb]{0.149,0.196,0.22}{Strength}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                 & \textcolor[rgb]{0.149,0.196,0.22}{Weakness}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                               &  &   \\
\begin{tabular}[c]{@{}l@{}}\textcolor[rgb]{0.149,0.196,0.22}{It is the first result regarding the one-failure structure}\\\textcolor[rgb]{0.149,0.196,0.22}{for all-pair s-t min-cut.}\\\textcolor[rgb]{0.149,0.196,0.22}{}\end{tabular}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                    & \begin{tabular}[c]{@{}l@{}}\textcolor[rgb]{0.149,0.196,0.22}{The major part of this paper is the description of}\\\textcolor[rgb]{0.149,0.196,0.22}{the linear space structure, but the query time of this structure is not so}\\\textcolor[rgb]{0.149,0.196,0.22}{efficient.}\\\\\textcolor[rgb]{0.149,0.196,0.22}{This paper is very well written. Maybe it will be better to move the O(n}\textcolor[rgb]{0.149,0.196,0.22}{2}\textcolor[rgb]{0.149,0.196,0.22}{)-space}\\\textcolor[rgb]{0.149,0.196,0.22}{and O(1)-query time structure in front since it is easier to comprehend.}\\\textcolor[rgb]{0.149,0.196,0.22}{}\end{tabular}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                &  &   \\
\begin{tabular}[c]{@{}l@{}}\textcolor[rgb]{0.149,0.196,0.22}{The paper makes progress on a fundamental question in algorithm design. While we}\\\textcolor[rgb]{0.149,0.196,0.22}{have witnessed a substantial number of works on fault-tolerant distance-based graph}\\\textcolor[rgb]{0.149,0.196,0.22}{approximations, not much was known about the higher-connectivity structure of graphs}\\\textcolor[rgb]{0.149,0.196,0.22}{in this setting.}\\\textcolor[rgb]{0.149,0.196,0.22}{Even though the techniques used in this paper may not feel very novel to someone}\\\textcolor[rgb]{0.149,0.196,0.22}{being fairly familiar with fault-tolerant data-structures and network flow theory,}\\\textcolor[rgb]{0.149,0.196,0.22}{the paper certainly does some non-trivial chunk of work to bring together the}\\\textcolor[rgb]{0.149,0.196,0.22}{Steiner min-cut representations and labelling schemes. Moreover, these}\\\textcolor[rgb]{0.149,0.196,0.22}{data-structures themselves are far from being easy to grasp.}\\\textcolor[rgb]{0.149,0.196,0.22}{The writing is clear and to the point.}\\\textcolor[rgb]{0.149,0.196,0.22}{}\end{tabular} & \begin{tabular}[c]{@{}l@{}}\textcolor[rgb]{0.149,0.196,0.22}{One obvious limitation is that the current data-structure supports only 1 edge}\\\textcolor[rgb]{0.149,0.196,0.22}{deletion. The fault-tolerant setting is considered to be more competitive when the data-structure supports up to K-edge deletions. This would be more exciting, as it is closer to maintaining all-pairs (s-t) min-cuts dynamically.}\\\textcolor[rgb]{0.149,0.196,0.22}{I find it strange that the paper does not discuss the preprocessing time of the}\\\textcolor[rgb]{0.149,0.196,0.22}{data-structure and only focuses on space complexity. I would assume that running}\\\textcolor[rgb]{0.149,0.196,0.22}{time is a more relevant parameter for this problem.~}\\\textcolor[rgb]{0.149,0.196,0.22}{Another concern regarding the paper is that in various settings this paper is only}\\\textcolor[rgb]{0.149,0.196,0.22}{providing query complexity improvements (of more than logarithmic factors) over}\\\textcolor[rgb]{0.149,0.196,0.22}{deterministic algorithms. In these cases, randomized solutions with the same query complexity (up to logarithmic factors) could be achieved just by applying}\\\textcolor[rgb]{0.149,0.196,0.22}{state-of-the-art randomized maximum flow / minimum s-t cut algorithms blackbox.}\\\textcolor[rgb]{0.149,0.196,0.22}{}\end{tabular} &  &   \\
\begin{tabular}[c]{@{}l@{}}\textcolor[rgb]{0.149,0.196,0.22}{The authors study a new problem of fault-tolerant all-pairs mincuts.}\\\textcolor[rgb]{0.149,0.196,0.22}{The authors develop two data-structures, one is query optimal (constant query time)}\\\textcolor[rgb]{0.149,0.196,0.22}{using O(n\^2) space, and the other is space optimal - O(m) space with a query}\\\textcolor[rgb]{0.149,0.196,0.22}{a procedure that is at least \textbackslash{}sqrt\{n\} times more efficient than the static algorithm.}\\\textcolor[rgb]{0.149,0.196,0.22}{The data-structures developed by the authors are interesting, innovative, and give a solid contribution to this field.}\\\textcolor[rgb]{0.149,0.196,0.22}{The main strength of this paper, in my opinion, is researching a new interesting}\\\textcolor[rgb]{0.149,0.196,0.22}{question and giving a sophisticated and efficient data-structure for this problem.}\\\textcolor[rgb]{0.149,0.196,0.22}{}\end{tabular}                                                                                                                                                                            & \begin{tabular}[c]{@{}l@{}}\textcolor[rgb]{0.149,0.196,0.22}{As there is no previous work on fault-tolerant mincuts, it is difficult to evaluate}\\\textcolor[rgb]{0.149,0.196,0.22}{the achievement of how efficient the query time is and how further can the query}\\\textcolor[rgb]{0.149,0.196,0.22}{time be improved. Is there any relevant conditional lower bound?}\\\textcolor[rgb]{0.149,0.196,0.22}{~}\textcolor[rgb]{0.149,0.196,0.22}{I think that the authors study an interesting problem, present a sophisticated and}\\\textcolor[rgb]{0.149,0.196,0.22}{clever solution, and this work may lead to additional research of fault-tolerant}\\\textcolor[rgb]{0.149,0.196,0.22}{mincuts. Also, the writeup is very good.~ Thus, I tend towards acceptance, with the}\\\textcolor[rgb]{0.149,0.196,0.22}{weakness that it is hard to evaluate their bounds without lower bounds of any kind.}\\\textcolor[rgb]{0.149,0.196,0.22}{}\end{tabular}                                                                                                                                                                                                                                                                                                                                                                                                             &  &  
\end{tabular}
\end{table}

==> src/todo.tex <==
{\color{blue} To do list:
\begin{enumerate}
% \item What is the best deterministic bound on computing
% $(s,t)$-mincut in an undirected unweighted graph ? We need this information to show the nontriviality of the query time of our second data structure.\\

% Case 1: $m>nv$

% 1. $nm^{2/3}v^{1/6} > n^{5/3}v^{5/6}$, therefore, 
% $\frac{nv}{n^{5/3}v^{5/6}} \leq \frac{1}{n^{1/2}}$

% 2. $n^{3/2}m^{1/2} > n^{2}v^{1/2}$, therefore, 
% $\frac{nv}{n^{2}v^{1/2}} \leq \frac{1}{n^{1/2}}$

% Case 2: $m<nv$

% 1. $nm^{2/3}v^{1/6} > n^{5/6}m^{5/6}$, therefore, 
% $\frac{m}{n^{5/6}m^{5/6}} \leq \frac{1}{n^{1/2}}$

% 2. $\frac{m}{n^{3/2}m^{1/2}} \leq \frac{1}{n^{1/2}}$

% Therefore, it gives a $\sqrt{n}$ factor of improvement in query time, using the best algorithms.

\item @Abhyuday: Now I fully agree with you that if we are able to build our data structure(s) in $O(mF)$ time, it will add more value to our results. So we must strive to accomplish this goal and provide all details in Appendix.
\item What is the best lower bound that we can achieve on the fault tolerant all-pairs mincuts data structures for a graph with edge capacities polynomial in $n$ if the desired query time is $O(1)$ or $O($polylog$(n))$?
\item Distributed memory and parallelize query.
\item Time taken to report a mincut in 1 and 2.
\item Proof of E.1 uses the construction of strip corresponding to subbunch in 2.2. Try to refer it somehow.
\item Streamline Appendix G.
\item Add other fault tolerant data structures.
\item multigraph.
\end{enumerate}}


{

\color{brown} Doubts
\begin{enumerate}
    \item DKL figure issue.
    \item Resolve Strip Lemma (ii) part.
    \item Path $(\nu_1,\nu_2)$ and $(\nu_3,\nu_4)$ extendable intuition?
\end{enumerate}
}

% Suppose $u$ is a stretched unit in the flesh ${\cal F}_S$. Suppose ${\cal R}_1$ and ${\cal R}_2$ denote its two reachability cones. Each of ${\cal R}_1$,${\cal R}_2$,${\cal R}_1\setminus \{u\}$ and ${\cal R}_2 \setminus \{u\}$ define a steiner mincut. This can be proved by showing that no coherent path can interesect any of the above sets twice.

% Since ${\cal R}_1$ is a steiner mincut, it must correspond to some subbunch, say ${\cal B}$, in the skeleton ${\cal H}_S$. Suppose the path to which $u$ is mapped in the skeleton be $P(\nu_1,\nu_2)$. We claim that the subcactus rooted at $\nu_1$ wrt to path $P(\nu_1,\nu_2)$ is the minimal cut in the skeleton that represents this subbunch. The reason for the same is as follows. Suppose ${\cal H}_S({\cal B})\subset {\cal H}_S(\nu_1)$. Then $u$ must appear as a non-terminal in the strip representing this subbunch (because ${\cal R}_1\setminus \{u\}$ must be from the same subbunch). However ${\cal H}_S({\cal B})\subset {\cal H}_S(\nu_1)$, therefore $u$ cannot be mapped to any of the edges corresponding to cut ${\cal H}_S({\cal B})$. Thus, we arrive at a contradiction.

% \begin{lemma}
% If a stretched unit $u$ is mapped to path $P(\nu_1,\nu_2)$ in the skeleton, then the set of terminals in the reachability cones ${\cal R}_1$ and ${\cal R}_2$ coincide with the subbunch ${\cal H}_S(\nu_1)$ and ${\cal H}_S(\nu_2)$.
% \end{lemma}

% Now, we can easily derive Lemma 17. Suppose $u'$ be any stretched unit, such that $u'\in {\cal R}_1$. Moreover, let ${\cal R}_1'$ and ${\cal R}_2'$ denote the reachability cones of $u'$ such that ${\cal R}_1'\subseteq {\cal R}_1$ and ${\cal R}_2 \subseteq {\cal R}_2'$. Observe that this implies that the $\nu_3 \in {\cal H}_S(\nu_1)$ and $\nu_2 \in {\cal H}_S(\nu_4)$.
